Exemplar VAE: Linking Generative Models, Nearest Neighbor Retrieval, and Data Augmentation

We introduce Exemplar VAEs, a family of generative models that bridge the gap between parametric and non-parametric, exemplar based generative models. Exemplar VAE is a variant of VAE with a non-parametric prior in the latent space based on a Parzen window estimator. To sample from it, one first draws a random exemplar from a training set, then stochastically transforms that exemplar into a latent code and a new observation. We propose retrieval augmented training (RAT) as a way to speed up Exemplar VAE training by using approximate nearest neighbor search in the latent space to define a lower bound on log marginal likelihood. To enhance generalization, model parameters are learned using exemplar leave-one-out and subsampling. Experiments demonstrate the effectiveness of Exemplar VAEs on density estimation and representation learning. Importantly, generative data augmentation using Exemplar VAEs on permutation invariant MNIST and Fashion MNIST reduces classification error from 1.17% to 0.69% and from 8.56% to 8.16%.

==> extras.tex <==

\newpage

\begin{table*}[t!]
\begin{tabular}{rcccccc}
\toprule
Method && K=3 & K=5 & K=7 & k=10 \\ 
\midrule
VAE w/ Gaussian prior  &&  $97.05$\footnotesize{$ \pm 0.22$} &  $97.21$\footnotesize{$ \pm 0.15$} & {\boldmath$97.23$}\footnotesize{$ \pm 0.14$} & $97.18$\footnotesize{$ \pm 0.16$} \\
VAE w/ VampPrior       &&  {\boldmath$98.32$}\footnotesize{$ \pm 0.03$} & $98.26$\footnotesize{$ \pm 0.03$} & $98.30$\footnotesize{$ \pm 0.04$} & $98.20$\footnotesize{$ \pm 0.08$} \\
Exemplar VAE           &&  $98.58$ \footnotesize{$ \pm 0.05$} & $98.61$\footnotesize{$\pm 0.07$} & {\boldmath$98.63$} \footnotesize{$ \pm 0.05$}& $98.6$\footnotesize{$ \pm 0.06$} \\
\midrule
HVAE w/ Gaussian prior && $95.24$\footnotesize{$ \pm 0.29$} & $95.65$\footnotesize{$ \pm 0.25$} & {\boldmath$95.82$} \footnotesize{$ \pm 0.16$} & $95.73$\footnotesize{$ \pm 0.13$}\\
HVAE w/ VampPrior  &&  $98.14$\footnotesize{$ \pm 0.09$} & $98.15$\footnotesize{$ \pm 0.06$} & {\boldmath $98.19$}\footnotesize{$ \pm 0.06$} & $98.07$\footnotesize{$ \pm 0.04$}  \\
Exemplar HVAE && $98.41$\footnotesize{$ \pm 0.08$} & $98.47$\footnotesize{$ \pm 0.07$} & {\boldmath $98.48$}\footnotesize{$ \pm 0.08$}&$98.44$\footnotesize{$ \pm 0.02$} \\
\midrule
ConvHVAE w/ Gaussian prior&& $95.24$ \footnotesize{$\pm0.73$}&{\boldmath$95.62$} \footnotesize{$\pm0.64$}&$95.58$ \footnotesize{$\pm0.61$}&$95.64$ \footnotesize{$\pm0.54$} \\
ConvHVAE w/ VampPrior && $98.16$ \footnotesize{$\pm0.48$}&{\boldmath$98.19$} \footnotesize{$\pm0.43$}&$98.16$ \footnotesize{$\pm0.47$}&$98.07$ \footnotesize{$\pm0.49$}  \\
Exemplar ConvHVAE &&  $98.74$ \footnotesize{$\pm0.13$}&{\boldmath$98.8$} \footnotesize{$\pm0.08$}&$98.76$ \footnotesize{$\pm0.07$}&$98.67$ \footnotesize{$\pm0.12$} \\
\bottomrule
\end{tabular}
\caption{Validation set classification accuracies of different models using KNN classifier on MNIST. For hierarchical versions we just use the higher level set of latent variables. We bolded the best number in each row.}
\label{tab:loglikelihoodA}
\end{table*}

\begin{table*}[t!]
\hspace*{-1cm}~\begin{tabular}{rcccccccc}
\toprule
Method && K=3 & K=5 & K=7 & k=9 & k=11 & k=13 & k=15\\ 
\midrule
VAE w/ Gaussian Prior && $82.09$ \footnotesize{$\pm0.51$}&$83.08$ \footnotesize{$\pm0.48$}&$83.49$ \footnotesize{$\pm0.45$}&$83.64$ \footnotesize{$\pm0.56$}&$83.73$ \footnotesize{$\pm0.42$}&{\boldmath$83.76$} \footnotesize{$\pm0.51$}&{\boldmath $83.76$} \footnotesize{$\pm0.44$} \\
VAE w/ Vampprior && $85.75$ \footnotesize{$\pm0.15$}&$86.32$ \footnotesize{$\pm0.21$}&$86.49$ \footnotesize{$\pm0.07$}&$86.5$ \footnotesize{$\pm0.13$}&$86.44$ \footnotesize{$\pm0.11$}&{\boldmath$86.52$} \footnotesize{$\pm0.14$}&$86.5$ \footnotesize{$\pm0.08$} \\
Exemplar VAE && $86.37$ \footnotesize{$\pm0.16$}&$86.91$ \footnotesize{$\pm0.08$}&$86.94$ \footnotesize{$\pm0.1$}&{\boldmath$87.04$} \footnotesize{$\pm0.13$}&$86.96$ \footnotesize{$\pm0.17$}&$86.97$ \footnotesize{$\pm0.12$}&$86.87$ \footnotesize{$\pm0.11$}\\
\midrule
HVAE w/ Gaussian Prior && $78.24$ \footnotesize{$\pm0.56$}&$79.74$ \footnotesize{$\pm0.59$}&$80.46$ \footnotesize{$\pm0.55$}&$80.83$ \footnotesize{$\pm0.45$}&$81.06$ \footnotesize{$\pm0.53$}&$81.2$ \footnotesize{$\pm0.57$}&{\boldmath$81.42$} \footnotesize{$\pm0.65$}\\
HVAE w/ Vampprior && $84.54$ \footnotesize{$\pm0.32$}&$85.26$ \footnotesize{$\pm0.41$}&$85.44$ \footnotesize{$\pm0.35$}&$85.5$ \footnotesize{$\pm0.41$}&$85.48$ \footnotesize{$\pm0.4$}&$85.51$ \footnotesize{$\pm0.45$}&{\boldmath $85.57$} \footnotesize{$\pm0.28$}  \\
Exemplar HVAE && $84.67$ \footnotesize{$\pm0.92$}&$85.14$ \footnotesize{$\pm0.82$}&$85.39$ \footnotesize{$\pm0.85$}&$85.53$ \footnotesize{$\pm0.82$}&$85.5$ \footnotesize{$\pm0.73$}&$85.55$ \footnotesize{$\pm0.78$}&{\boldmath $85.58$} \footnotesize{$\pm0.82$}\\
\midrule
ConvHVAE w/ Gaussian Prior && $78.17$ \footnotesize{$\pm1.29$}&$79.64$ \footnotesize{$\pm1.12$}&$80.19$ \footnotesize{$\pm1.03$}&$80.49$ \footnotesize{$\pm0.93$}&$80.65$ \footnotesize{$\pm0.79$}&$80.67$ \footnotesize{$\pm0.96$}&{\boldmath$80.75$} \footnotesize{$\pm0.98$} \\
ConvHVAE w/ Vampprior && $84.6$ \footnotesize{$\pm0.54$}&$85.18$ \footnotesize{$\pm0.46$}&$85.68$ \footnotesize{$\pm0.12$}&$85.6$ \footnotesize{$\pm0.25$}&$85.56$ \footnotesize{$\pm0.16$}&{\boldmath$85.57$} \footnotesize{$\pm0.2$}&$85.54$ \footnotesize{$\pm0.19$}  \\
Exemplar ConvHVAE && $85.46$ \footnotesize{$\pm0.54$}&$85.99$ \footnotesize{$\pm0.43$}&$86.03$ \footnotesize{$\pm0.43$}&$86.1$ \footnotesize{$\pm0.49$}&$86.15$ \footnotesize{$\pm0.4$}&\boldmath{$86.15$} \footnotesize{$\pm0.49$}&$86.02$ \footnotesize{$\pm0.47$}
\end{tabular}
\caption{Validation set classification accuracies of different models using KNN classifier on Fashion-MNIST. For hierarchical versions we just use the higher level set of latent variables}
\label{tab:loglikelihoodB}
\end{table*}


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/interpolations.png}
\end{center}
\label{figure:mnist_generationC}
\caption{}
\end{figure}



\newpage



